Completely regular codes in the infinite hexagonal grid

A set $C$ of vertices of a simple graph is called a completely regular code if for each $i=0$, $1$, $2$, \ldots and $j = i-1$, $i$, $i+1$, all vertices at distance $i$ from $C$ have the same number $s_{ij}$ of neighbors at distance $j$ from $C$. We characterize the completely regular codes in the infinite hexagonal grid graph.

==> 03-111-12.tex <==
\def\uo{\ucolor{white}{$\ $}}
\def\do{\dcolor{white}{$\ $}}
\def\ua{\ucolor{yellow!20!white}{$0$}}
\def\da{\dcolor{yellow!20!white}{$0$}}
\def\ub{\ucolor{yellow!60!white}{$1$}}
\def\db{\dcolor{yellow!60!white}{$1$}}
\def\0{++(1,0)}
\def\uc{\ucolor{orange!65!white}{$2$}}
\def\dc{\dcolor{orange!65!white}{$2$}}
\def\ud{\ucolor{red!85!brown!70!white}{$3$}}
\def\dd{\dcolor{red!85!brown!70!white}{$3$}}
\def\ue{\ucolor{brown!80!black}{$4$}}
\def\de{\dcolor{brown!80!black}{$4$}}
\begin{tikzpicture}[scale=0.65, rotate=-90]
\draw (0, 6.928)\da\ub\dc\uc\db\ub\dc\uc\db;
\draw (0, 5.192)\ub\dc\uc\db\ua\db\uc\dc\ub;
\draw (0, 3.464)\db\uc\dc\ub\da\ub\dc\uc\db;
\draw (0, 1.732)\ub\dc\uc\db\ub\dc\uc\db\ua;
\draw (0,-0.000)\dc\uc\db\ua\db\uc\dc\ub\da;
\draw (0,-1.732)\uc\dc\ub\da\ub\dc\uc\db\ub;
\draw (0,-3.464)\dc\uc\db\ub\dc\uc\db\ua\db;
\draw (0,-5.192)\uc\db\ua\db\uc\dc\ub\da\ub;
\draw (0,-6.928)\dc\ub\da\ub\dc\uc\db\ub\dc;
\draw (0,-8.660)\uc\db\ub\dc\uc\db\ua\db\uc;
\end{tikzpicture}


==> 21-111--111-21fin1.tex <==
\def\ut{ ++(1, 0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0,-0.29) }%
\def\dt{ ++(1,-0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0, 0.29) }%
\def\uo{\ucolor{white}{$\ $}}%
\def\do{\dcolor{white}{$\ $}}%
\def\ux{\ucolor{white}{$$}}%
\def\dx{\dcolor{white}{$$}}%
\def\ua{\ucolor{yellow!20!white}{$0$}}%
\def\da{\dcolor{yellow!20!white}{$0$}}%
\def\ub{\ucolor{yellow!60!white}{$1$}}%
\def\db{\dcolor{yellow!60!white}{$1$}}%
\def\0{++(1,0)}%
\def\uc{\ucolor{orange!65!white}{$2$}}%
\def\dc{\dcolor{orange!65!white}{$2$}}%
\def\ud{\ucolor{red!85!brown!70!white}{$3$}}%
\def\dd{\dcolor{red!85!brown!70!white}{$3$}}%
\def\ue{\ucolor{brown!80!black}{$\ $}}%
\def\de{\dcolor{brown!80!black}{$\ $}}%
\def\uf{\ucolor{black}{$\ $}}%
\def\df{\dcolor{black}{$\ $}}%
\begin{tikzpicture}[scale=0.65, rotate=-90]
\draw (0, 5.192) \db\ua\da\ub\dc\dt\de\uf\df\ue\dt\dc\db\ua\da\ub;
\draw (0, 3.464) \ub\da\ua\db\uc\0 \ue\df\uf\de\0 \uc\ub\da\ua\db;
\draw (0, 1.732) \db\ua\da\ub\dc\dt\de\uf\df\ue\dt\dc\db\ua\da\ub;
\draw (0,-0.000) \ub\da\ua\db\uc\0 \ue\df\uf\de\0 \uc\ub\da\ua\db;
\draw (0,-1.732) \db\ua\da\ub\dc\dt\de\uf\df\ue\dt\dc\db\ua\da\ub;
\draw (0,-3.464) \ub\da\ua\db\uc\0 \ue\df\uf\de\0 \uc\ub\da\ua\db;
\draw (0,-5.192) \db\ua\da\ub\dc\dt\de\uf\df\ue\dt\dc\db\ua\da\ub;
\draw (0,-6.928) \ub\da\ua\db\uc\0 \ue\df\uf\de\0 \uc\ub\da\ua\db;
\draw (0,-8.660) \db\ua\da\ub\dc\dt\de\uf\df\ue\dt\dc\db\ua\da\ub;
\end{tikzpicture}

==> 21-111--111-21fin2.tex <==
\def\ut{ ++(1, 0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0,-0.29) }%
\def\dt{ ++(1,-0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0, 0.29) }%
\def\uo{\ucolor{white}{$\ $}}%
\def\do{\dcolor{white}{$\ $}}%
\def\ux{\ucolor{white}{$$}}%
\def\dx{\dcolor{white}{$$}}%
\def\ua{\ucolor{yellow!20!white}{$0$}}%
\def\da{\dcolor{yellow!20!white}{$0$}}%
\def\ub{\ucolor{yellow!60!white}{$1$}}%
\def\db{\dcolor{yellow!60!white}{$1$}}%
\def\0{++(1,0)}%
\def\uc{\ucolor{orange!65!white}{$2$}}%
\def\dc{\dcolor{orange!65!white}{$2$}}%
\def\ud{\ucolor{red!85!brown!70!white}{$3$}}%
\def\dd{\dcolor{red!85!brown!70!white}{$3$}}%
\def\ue{\ucolor{brown!80!black}{$\ $}}%
\def\de{\dcolor{brown!80!black}{$\ $}}%
\def\uf{\ucolor{black}{$\ $}}%
\def\df{\dcolor{black}{$\ $}}%
\begin{tikzpicture}[scale=0.65, rotate=-90]
\draw (0, 5.192) \db\ua\da\ub\dc\dt\ue\df\uf\de\dt\dc\db\ua\da\ub;
\draw (0, 3.464) \ub\da\ua\db\uc\0 \de\uf\df\ue\0 \uc\ub\da\ua\db;
\draw (0, 1.732) \db\ua\da\ub\dc\dt\ue\df\uf\de\dt\dc\db\ua\da\ub;
\draw (0,-0.000) \ub\da\ua\db\uc\0 \de\uf\df\ue\0 \uc\ub\da\ua\db;
\draw (0,-1.732) \db\ua\da\ub\dc\dt\ue\df\uf\de\dt\dc\db\ua\da\ub;
\draw (0,-3.464) \ub\da\ua\db\uc\0 \de\uf\df\ue\0 \uc\ub\da\ua\db;
\draw (0,-5.192) \db\ua\da\ub\dc\dt\ue\df\uf\de\dt\dc\db\ua\da\ub;
\draw (0,-6.928) \ub\da\ua\db\uc\0 \de\uf\df\ue\0 \uc\ub\da\ua\db;
\draw (0,-8.660) \db\ua\da\ub\dc\dt\ue\df\uf\de\dt\dc\db\ua\da\ub;
\end{tikzpicture}

==> abcde-.tex <==
\def\0{++(1,0)}%
\def\uo{\ucolor{white}{$\ $}}%
\def\do{\dcolor{white}{$\ $}}%
\def\dxa{\dcolor{white}{$\boldsymbol a$}}%
\def\uxa{\ucolor{white}{$\boldsymbol a$}}%
\def\dxb{\dcolor{white}{$\boldsymbol b$}}%
\def\uxb{\ucolor{white}{$\boldsymbol b$}}%
\def\ua#1{\ucolor{yellow!60!white}{$0_{\mathrm #1}$}}%
\def\da#1{\dcolor{yellow!60!white}{$0_{\mathrm #1}$}}%
\def\ub#1{\ucolor{orange!65!white}{$1_{\mathrm #1}$}}%
\def\db#1{\dcolor{orange!65!white}{$1_{\mathrm #1}$}}%
\def\uc#1{\ucolor{red!85!brown!70!white}{$2_{\mathrm #1}$}}%
\def\dc#1{\dcolor{red!85!brown!70!white}{$2_{\mathrm #1}$}}%
\def\ud#1{\ucolor{brown!80!black}{$3_{\mathrm #1}$}}%
\def\dd#1{\dcolor{brown!80!black}{$3_{\mathrm #1}$}}%
\def\Ua#1{\Ucolor{yellow!60!white}{$0_{\mathrm #1}$}}%
\def\Da#1{\Dcolor{yellow!60!white}{$0_{\mathrm #1}$}}%
\def\Ub#1{\Ucolor{orange!65!white}{$1_{\mathrm #1}$}}%
\def\Db#1{\Dcolor{orange!65!white}{$1_{\mathrm #1}$}}%
\def\Uc#1{\Ucolor{red!85!brown!70!white}{$2_{\mathrm #1}$}}%
\def\Dc#1{\Dcolor{red!85!brown!70!white}{$2_{\mathrm #1}$}}%
\def\Ud#1{\Ucolor{brown!80!black}{$3_{\mathrm #1}$}}%
\def\Dd#1{\Dcolor{brown!80!black}{$3_{\mathrm #1}$}}%
\def\ut{ ++(1, 0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0,-0.29) }%
\def\dt{ ++(1,-0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0, 0.29) }%
\def\uU{ ++(1,-0.87) node  {\raisebox{-0.15em}[0.2em][0em]{\makebox[0mm][c]{$*$}}} ++(-1,0.87) }%

==> abcde0-.tex <==
\def\0{++(1,0)}%
\def\uo{\ucolor{white}{$\ $}}%
\def\do{\dcolor{white}{$\ $}}%
\def\ua{\ucolor{yellow!60!white}{$0$}}%
\def\da{\dcolor{yellow!60!white}{$0$}}%
\def\ub{\ucolor{orange!65!white}{$1$}}%
\def\db{\dcolor{orange!65!white}{$1$}}%
\def\uc{\ucolor{red!85!brown!70!white}{$2$}}%
\def\dc{\dcolor{red!85!brown!70!white}{$2$}}%
\def\ud{\ucolor{brown!80!black}{$3$}}%
\def\dd{\dcolor{brown!80!black}{$3$}}%
\def\Ua{\Ucolor{yellow!60!white}{$0$}}%
\def\Da{\Dcolor{yellow!60!white}{$0$}}%
\def\Ub{\Ucolor{orange!65!white}{$1$}}%
\def\Db{\Dcolor{orange!65!white}{$1$}}%
\def\Uc{\Ucolor{red!85!brown!70!white}{$2$}}%
\def\Dc{\Dcolor{red!85!brown!70!white}{$2$}}%
\def\Ud{\Ucolor{brown!80!black}{$3$}}%
\def\Dd{\Dcolor{brown!80!black}{$3$}}%
\def\ut{ ++(1, 0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0,-0.29) }%
\def\dt{ ++(1,-0.29) node  {\raisebox{-0.25em}[0.2em][0em]{\makebox[0mm][c]{$\cdots$}}}  ++(0, 0.29) }%
\def\uU{ ++(1,-0.87) node  {\raisebox{-0.15em}[0.2em][0em]{\makebox[0mm][c]{$*$}}} ++(-1,0.87) }%
